Model-based Deep Learning for QoS-Aware Rate-Splitting Multiple Access Wireless Systems

Next generation communications demand for better spectrum management, lower latency, and guaranteed quality-of-service (QoS). Recently, Artificial intelligence (AI) has been widely introduced to advance these aspects in next generation wireless systems. However, such AI applications suffer from limited training data, low robustness, and poor generalization capabilities. To address these issues, a model-driven deep unfolding (DU) algorithm is introduced in this paper to bridge the gap between traditional model-driven communication algorithms and data-driven deep learning. Focusing on the QoS-aware rate-splitting multiple access (RSMA) resource allocation problem in multi-user communications, a conventional fractional programming (FP) algorithm is first applied as a benchmark. The solution is then refined by the application of projection gradient descent (PGD). DU is employed to further speed up convergence procedure, hence improving the efficiency of PGD. Moreover, the feasibility of results is guaranteed by designing a low-complexity projection based on scale factors, plus adding violation control mechanisms into the loss function that minimizes error rates. Finally, we provide a detailed analysis of the computational complexity and analysis design of the proposed DU algorithm. Extensive simulations are conducted and the results demonstrate that the proposed DU algorithm can reach the optimal communication efficiency with a mere $0.024\%$ violation rate for 4 layers DU. The DU algorithm also exhibits robustness in out-of-distribution tests and can be effectively trained with as few as 50 samples.

==> difference.tex <==
\begin{document}

This journal article builds upon the foundational work presented in the conference paper, which focused on model-based deep learning for resource allocation in an RSMA (Rate-Splitting Multiple Access) wireless system. The journal version introduces several critical enhancements and methodological advancements that go beyond the initial scope of the conference version. These differences can be summarized as follows:

\begin{enumerate}
    \item \textbf{Enhanced Problem Complexity}: 
        \begin{itemize}
            \item The conference paper tackled a relatively simple resource allocation problem, allowing for a basic deep unfolding design with a straightforward learning approach.
            \item In contrast, the journal version addresses a more complex problem by considering the Quality of Service (QoS) requirements for each user's data rate. This added constraint necessitates a more sophisticated approach to ensure that each user meets their specific data rate needs within the RSMA framework.
        \end{itemize}
        
    \item \textbf{Advanced Optimization Techniques}:
        \begin{itemize}
            \item To resolve the QoS constraints introduced in the journal version, a projected gradient descent method is applied. This method enables the model to handle additional constraints effectively, maintaining an efficient resource allocation that meets users' requirements.
            \item The incorporation of projected gradient descent marks a significant methodological improvement, as it ensures adherence to QoS standards within a more constrained optimization landscape.
        \end{itemize}
        
    \item \textbf{Extended Performance Analysis}:
        \begin{itemize}
            \item The journal article includes an extensive analysis of model performance, expanding on results presented in the conference version.
            \item This performance analysis covers several new dimensions, including a complexity analysis to assess computational feasibility, comparisons with traditional data-driven learning approaches to benchmark effectiveness, and an in-depth violation rate analysis, which examines the frequency and severity of constraint violations in real-world scenarios.
            \item These additional evaluations provide a comprehensive understanding of the model’s operational behavior, offering insights into its potential for practical applications in RSMA systems.
        \end{itemize}
\end{enumerate}

These improvements make the journal version a considerably more robust and detailed study, offering valuable insights into the practical implementation of model-based deep learning for resource allocation in RSMA wireless systems. The extended results and refined methodologies presented in the journal contribute significantly to advancing the field and highlight the potential for model-based deep learning in resource-constrained, QoS-aware wireless environments.

\end{document}
